Digraphs modulo primitive positive constructability

This is my dissertation about digraphs ordered by pp-constructability. We study in particular smooth digraphs, i.e., digraphs without sources or sinks, tournaments and semicomplete digraphs, orientations of paths and cycles, digraphs with at most four vertices, and orientations of trees.

==> 11_finiteDualityTrash.tex <==

\begin{theorem}\label{thm:Datalog}
\begin{enumerate}
    \item if $\cocsp(\A)$ is in Datalog, then $\csp(\A)$ is in P,
    \item $\cocsp(\A)$ is in Datalog if and only if $\A\models 34WNU$
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:linearDatalog}
\begin{enumerate}
    \item if $\cocsp(\A)$ is in linear Datalog, then $\csp(\A)$ is in NL,
    \item $\cocsp(\A)$ is in linear Datalog if and only if $\A$ has bounded pathwidth duality
    \item if $\A\models Jonnson n$ for some $n\geq1$, then $\cocsp(\A)$ in linear Datalog
    \item if $\A\models \NU n$ for some $n\geq3$, then $\cocsp(\A)$ is in linear Datalog 
    \item if $\A\not\models\KK n$ for all $n\geq2$, then $\cocsp(\A)$ is not in linear Datalog,
    \item $\NN n$
    
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:treeDatalog}
\begin{enumerate}
    \item if $\cocsp(\A)$ is in tree Datalog, then $\csp(\A)$ is in P,
    \item $\cocsp(\A)$ is in tree Datalog if and only if $\A\models \TS n$ for all $n\geq1$,
    \item $\cocsp(\A)$ is in tree Datalog if and only if $\A$ has tree duality,
    \item $\cocsp(\A)$ is in tree Datalog if and only if $\cocsp(\A)$ is solved by the arc-consistency procedure,
\end{enumerate}
\end{theorem}

\begin{theorem}\label{thm:symmetricLinearDatalog}
\begin{enumerate}
    \item if $\cocsp(\A)$ is in symmetric linear Datalog, then $\csp(\A)$ is in L,
    \item if $\A\models\HM n$ for some $n\geq1$ and $\cocsp(\A)$ in linear Datalog, then $\cocsp(\A)$ in symmetric linear Datalog
    \item symmetric linear Datalog is the intersection of linear Datalog and symmetric Datalog (why?, whats with the others?)
\end{enumerate}
\end{theorem}


\begin{conjecture}
    if $\A\models\HM n$ for some $n\geq1$ and $\cocsp(\A)$ in Datalog, then $\cocsp(\A)$ in symmetric Datalog
\end{conjecture}

\begin{theorem}\label{thm:DatalogOverview}
Then
\begin{enumerate}
    \item if $\cocsp(\A)$ is in Datalog, then $\csp(\A)$ is in P,
    \item if $\cocsp(\A)$ is in linear Datalog, then $\csp(\A)$ is in NL,
    \item if $\cocsp(\A)$ is in linear symmetric Datalog, then $\csp(\A)$ is in L,
    \item  $\cocsp(\A)$ is in Datalog iff $\A\not\ppleq 3Lin_p$ for all $p$ iff $\A\models34WNU$
    \item if $\A\models Jonnson n$ for some $n\geq1$, then $\cocsp(\A)$ in linear Datalog
    \item if $\A\models \NU n$ for some $n\geq3$, then $\cocsp(\A)$ in linear Datalog y
    \item if $\A\models\HM n$ for some $n\geq1$ and $\cocsp(\A)$ in linear Datalog, then $\cocsp(\A)$ in symmetric linear Datalog
    \item if $\A\not\models\KK n$ for all $n\geq2$, then $\cocsp(\A)$ is not in linear Datalog,
    \item $\NN n$
    
    \item $\A\not\models\KK n$ for all $n\geq2$ iff $\A\ppleq Horn-3SAT$ or $\A\ppleq 3Lin_p$ for some $p$. In particular $\cocsp(\A)$ is not in linear Datalog. TODO check this and rewrite it and maybe remove 3Linp 
    \item $\cocsp(\Ord)$ is in linear Datalog but not in linear symmetric Datalog  
\end{enumerate}
\end{theorem}

\begin{proof}
(1) Theorem ?? in ??
(2) ....
\end{proof}




%_________________________________________________________________________




Sym Datalog, Linear Datalog, AC = Tree Datalog

\begin{lemma}
$\csp(\A)$ is solved by unary linear symmetric arc Datalog iff $\P_2\ppleq\A$.
\end{lemma}


\begin{lemma}
unary linear symmetric 2-arc Datalog is closed under pp-constructions
\end{lemma}

combining properties of dualities

\begin{conjecture}
$\G\in \operatorname{PP(FD)}$ if and only if $\overline{\operatorname{Dual}(\G)}$ has finite generating set in $\overline{\operatorname{Graphs},homorder}$, i.e. $\operatorname{Dual}(\G)$ consists of finitely many hom chains (of trees? or does this already follow). 
\end{conjecture}

\begin{lemma}
Let $A$ and $B$ be properties that are closed under taking cores $\csp$ has $A$-duality and $B$-duality implies $\csp$ has ($A$ and $B$)-duality (eg $A=$ finite, $B=$ tree)
\end{lemma}

\begin{lemma}
\begin{enumerate}
    \item PP(FO) implies tree duality  (ts(n) for all n)
    \item PP(FO) implies bounded path width duality (exists  NU(n))
    \item PP(FO) implies exists $\HM{n}$ 
\end{enumerate}
\end{lemma}
\begin{proof}
1)FO=>tree duality => ts(n)

2)FO <=> finite duality => bounded path width => NU 

3)Sei A in FO und A pp-constructs st-Con. OBdA ist die power der konstruktion 1  (vorher konstanten zu A hinzufügen) Sei phi(x,y) die pp-formel

betrachte instanzen von st-Con 1-> ->....... -> -> 0 und übersetzte sie mit der pp-formel in instanzen von A.

Da A finite duality hat muss die pp-formel = benutzen. also phi(x,y)="x=y" AND ......

Dann gilt aber phi(a,b) gdw phi(b,a) also 1<- <-....... <- <- 0 würde auch als negative instanz erkannt werden 
\end{proof}

\begin{lemma}
for every tree $\T$ there exists a graph $\G$ such that $\Dual{G}=\langle\T\rangle$
\end{lemma}
\begin{proof}
manuels, $V(\G)=2^{some rooted subtrees of \T}= P(\{(v,\T')\mid v\in \T,\T'\setminus v is a component of \T\setminus v\})$ 
$U\toEdge W$ iff 
\begin{itemize}
    \item there are no $u,w$ such that $u\toEdge w$ and all $(u,\T')$ with $w\notin \T'$ are in $U$ and all $(w,\T')$ with $u\notin \T'$ are in $W$.
    %\item there is no edge from $u\in V(\T without leafs)\setminus  U$ to some $w\in W$, and
    %\item there is no edge from $u\in U$ to some $w\in V(\T)\setminus W$ and
    %\item no out-leaf in $W$ and
    %\item no in-leaf in $U$
\end{itemize}

$I\to \G$ $x\mapsto \{(v,\T')\mid (v,\T') \to (x,I)\}$

\begin{lemma}
$\A$ is in PPFinD iff $\overline{\csp(\A)}=Forb(F)$ for some possibly infinite set $F$. where $F$ ordered by the homomorphism order consists of only finitel many chains
\end{lemma}

\end{proof}

==> 9_subsubmaximal.tex <==
\chapter{Subsubmaximal elements initial results}\label{cha:subsubmax}

put this after submaximal?

GFSn (ohne FS?)

\begin{lemma}
$\G\models G_n$ iff $\G$ is $n$-fenced (compare braided), i.e., for every $n$ paths, where the $k$th path has a zigzag at the $k$th edge, there is a direct path $P$ in $G$ and if all startpoints are the same $a\in\G$, then $P$ can be choosen such that $P$ starts in $a$, same for endpoint. 
\end{lemma}

no characterization, see $\C_2\not\models G_2$ also $G_2 \not\Rightarrow G_3$

but $G_2 \Rightarrow HM_n$

==> AllH1ids.tex <==
\section{All minor conditions?}\label{sec:allh1Conditions}

TODO sloppy here with function and functionsymbol


\begin{definition}\label{def:hm} 
For $n \geq 1$, the \emph{Hagemann-Mitschke condition of length $n$}, called $\HM n$, consists of the identities %a sequence of ternary operations  $p_1,\dots,p_{n}$ on $D$ that satisfy
\begin{align*}
p_1(x,x,x) & \approx p_1(x,y,y) \\
p_{i}(x,x,y) & \approx p_{i+1}(x,y,y) && \text{ for all } i \in \{1,\dots,n-1\} \\
p_n(x,x,y) & \approx p_n(y,y,y).
\end{align*}
\end{definition}

\begin{definition}
An operation $s_n \colon D^n \to D$ is called \emph{symmetric} if the operation $s_n$ satisfies 
\[s_n(x_1,\dots,x_{n-1},x_n) \approx s_n(x_2,\dots,x_n,x_1).\]
The respective height one condition is abbreviated by $\Sigma_n$. 
\end{definition}

\begin{definition}
An operation $s_n \colon D^n \to D$ is called \emph{fully symmetric} if  the operation $s_n$ satisfies 
\begin{align*}
    s_n(x_1,x_2,\dots,x_n) &\approx s_n(x_n,x_1,\dots,x_{n-1})\\
    s_n(x_1,x_2,\dots,x_n) &\approx s_n(x_2,,x_1\dots,x_n).
\end{align*}
The respective height one condition is abbreviated by $\operatorname{FS}(n)$. 
\end{definition}

\begin{definition}
An operation $s_n \colon D^n \to D$ is called \emph{totally symmetric} if for all variables
$x_1,\dots,x_n$ and $y_1,\dots,y_n$ such that $\{x_1,\dots,x_n\} = \{y_1,\dots,y_n\}$ the operation $s_n$ satisfies 
\[s_n(x_1,\dots,x_n) \approx s_n(y_1,\dots,y_n).\]
The respective height one condition is abbreviated by $\TS(n)$. 
\end{definition}

\begin{definition}
A \emph{Hobby-McKenzie chain} of length $n$ consists of ternary operations $d_0,\dots,d_n,p,e_0,\dots,e_n$
such that 
\begin{align*}
    d_0(x,y,z) & \approx x \\
    d_i(x,y,y) & \approx d_{i+1}(x,y,y) & \text{for even } i < n \\
    d_i(x,x,y) & \approx d_{i+1}(x,x,y) & \text{for odd } i < n \\
    d_i(x,y,x) & \approx d_{i+1}(x,y,x) & \text{for odd } i < n \\
    d_n(x,y,y) & \approx p(x,y,y) \\
    p(x,x,y) & \approx e_0(x,x,y) \\
    e_i(x,y,y) & \approx e_{i+1}(x,y,y) & \text{for even } i < n \\
    e_i(x,x,y) & \approx e_{i+1}(x,x,y) & \text{for odd } i < n \\
    e_i(x,y,x) & \approx e_{i+1}(x,y,x) & \text{for even } i < n \\
    e_n(x,y,z) & \approx z.
\end{align*}
\end{definition}
The respective height one condition is abbreviated by $\HMcK(n)$.

\begin{definition}%[from Theorem 9.11 in~\cite{HobbyMcKenzie}] \label{def:kk}
Let $D$ be a set. A \emph{Kearnes-Kiss chain of length
$n \geq 2$ over $D$} is a sequence
of ternary operations  $d_0,d_1,\dots,d_n$ on $D$ such that 
\begin{align*}
d_0(x,y,z) & \approx x \\
d_i(x,y,y) & \approx d_{i+1}(x,y,y) && \text{ for even } i \in \{0,1,\dots,n-1\} 
\\ 
d_i(x,y,x) & \approx d_{i+1}(x,y,x) 
&& \text{ for even } i \in \{0,1,\dots,n-1\} \\
d_i(x,x,y) & \approx d_{i+1}(x,x,y) && \text{ for odd } i  \in \{1,\dots,n-1\} \\
d_n(x,y,z) & \approx z .
\end{align*}
The respective height one condition is abbreviated by $\KK(n)$.
\end{definition}
Note that $\KK(n)$ implies $\KK(n+1)$ for every $n \geq 0$.  
Also note that the existence of a J{\'o}nsson chain implies the existence of a Kearnes-Kiss chain \cite{HobbyMcKenzie}; namely $
\J(n)$ trivially implies $\KK(2n+4)$.



\begin{definition}%[\cite{HobbyMcKenzie}, Theorem 9.15]\label{def:nn} 
For $n \geq 0$, a \emph{Noname chain of length $n$ over $D$} is a sequence
of operations  $f_0,f_1,\dots,f_n$ of arity four on $D$ such that 
\begin{align*}
f_0(x,y,y,z) & \approx x \\
f_i(x,x,y,x) & \approx f_{i+1}(x,y,y,x) && \text{for all } i \in \{0,\dots,n-1\} \\
f_i(x,x,y,y) & \approx f_{i+1}(x,y,y,y)
&& \text{for all } i \in \{0,\dots,n-1\} \\
f_n(x,x,y,z) & \approx z. 
\end{align*}
The respective height one condition is abbreviated by $\NN(n)$.
\end{definition}
Note that $\NN(n)$ implies $\NN(n+1)$ for every $n \geq 0$.


%cyclic conditions

%GFS conditions

%picture of all conditions? or just a list of all the implications

%_________________________________________________________________

\begin{definition}\label{def:jonsson} 
For $n \geq 0$, a sequence
of ternary operations  $j_1,j_2,\dots,j_{2n+1}$ is called a  \emph{J\'onsson chain of length $n$} if it  
satisfies the following height-one condition $\J(n)$:
\begin{align*}
x & \approx j_1(x,x,y) \\
j_{2i-1}(x,y,y) & \approx j_{2i}(x,y,y) && \text{ for all } i \in \{1,\dots,n\} \\
j_i(x,y,x) & \approx x && \text{ for all } i \in \{1,\dots,2n+1\} \\
j_{2i}(x,x,y) & \approx j_{2i+1}(x,x,y) && \text{ for all } i  \in \{1,\dots,n\} \\
j_{2n+1}(x,y,y) & \approx y.
\end{align*}
\end{definition}


\begin{definition}\label{def:wnu}
An operation $f$ of arity $k$, for $k \geq 2$, is called \emph{$k$-ary weak near-unanimity} (short, \emph{$k$-wnu}) if it satisfies the following  height-one condition $\operatorname{WNU}_k$: 
\begin{align*}
f(y,x,\dots,x) \approx f(x,y,x,\dots,x) \approx \cdots \approx f(x,\dots,x,y)
\end{align*}
\end{definition}

\begin{definition}\label{def:wnu34}
A pair of operations $f,g$ (short, \emph{3-4 WNU}) such that $f$ is a 3-wnu, $g$ is a 4-wnu, is called \emph{3-4 weak near-unanimity} if they additionally satisfy the identity
\[f(x,x,y) \approx g(x,x,x,y)\]
\end{definition}

\subsection{Sigger-conditions}

\begin{definition}
A $6$-ary operation $s$ is called \emph{Siggers} if it satisfies the height-one condition $\Siggers_6$:
\begin{align*}
s(a,a,b,b,c,c)\approx s(b,c,a,c,a,b)
\end{align*}
\end{definition}

\begin{definition}
A $4$-ary operation $s$ is called \emph{Siggers} if it satisfies the height-one condition $\Siggers_4$:
\begin{align*}
s(a,r,e,a)\approx s(r,a,r,e)
\end{align*}
\end{definition}


\begin{definition}
A pair of ternary operations $p,q$ is called \emph{Kearnes-Markovi\'{c}-McKenzie} if it satisfies the height-one condition $\Siggers_3$:
\begin{align*}
p(x,y,y) &\approx q(y,x,x)\approx q(x,x,y)\\
p(x,y,x)&\approx q(x,y,x).
\end{align*}


\end{definition}
